Enterprise Software Service Emulation: Constructing Large-Scale Testbeds

Constructing testbeds for systems which are interconnected with large networks of other software services is a challenging task. It is particularly difficult to create testbeds facilitating evaluation of the non-functional qualities of a system, such as scalability, that can be expected in production deployments. Software service emulation is an approach for creating such testbeds where service behaviour is defined by emulate-able models executed in an emulation runtime environment. We present (i) a meta-modelling framework supporting emulate-able service modelling (including messages, protocol, behaviour and states), and (ii) Kaluta, an emulation environment able to concurrently execute large numbers (thousands) of service models, providing a testbed which mimics the behaviour and characteristics of large networks of interconnected software services. Experiments show that Kaluta can emulate 10,000 servers using a single physical machine, and is a practical testbed for scalability testing of a real, enterprise-grade identity management suite. The insights gained into the tested enterprise system were used to enhance its design.

==> Makefile <==
############################################################################

# Makefile for ICSE 2016 Workshop submission

############################################################################

BIBTEX	  = bibtex
PDFLATEX  = pdflatex
UMASK	  = umask 027

MAINBASE  = HineEmulation2016
BIBFILES  = caise-2013.bib
MAINTEX	  = $(MAINBASE).tex
PDFTARGET = $(MAINBASE).pdf

MAKEFILE  = Makefile

SRCS	  = $(MAINBASE).tex abstract.tex introduction.tex \
		industry-scenario.tex approach.tex evaluation.tex \
		related-work.tex conclusion.tex

############################################################################

.SUFFIXES:	.tex .pdf

# pdf
pdf $(PDFTARGET) : $(SRCS) $(BIBFILES)
	@$(MAKE) pdfagain
	@$(MAKE) bib
	@$(MAKE) pdfagain
	@$(MAKE) pdfagain
	@$(MAKE) pdfagain
	@$(MAKE) pdfagain

# pdflatex only
pdfagain :
	@echo "pdflatex $(MAINBASE)"
	@( $(UMASK); $(PDFLATEX) $(MAINBASE) )

# # bibtex only
bib : $(BIBFILES)
	@( $(UMASK); $(BIBTEX) $(MAINBASE) )


# remove unnecessary files
clean :
	$(RM) *.aux *.log *.dvi *.out
	$(RM) *.blg *.bbl *.toc* *.lof *.lot
	$(RM) *~ 
	$(RM) $(PDFTARGET)

############################################################################


==> background.tex <==
\section{Background} % May not be the best name for this
% section. Perhaps just call it 'motivating example'?

\cmh{Is this section necessary?}

\paragraph*{CA Identity Minder}\ph\\ % OUTLINE

\paragraph*{Required Test-Bed for Non-Functional Testing of Identity Minder}\ph\\ % OUTLINE

\paragraph*{Fruitless Hypothetical Attempts with Existing Approaches}\ph\\ % OUTLINE

\paragraph*{Reiterate Limitations in IM context}\ph\\ % OUTLINE

\paragraph*{Requirements for Ideal Solution}\ph\\ % OUTLINE

\paragraph*{Potential Impact of Ideal Solution}\ph\\ % OUTLINE

\subsection{LDAP Directories} % OUTLINE
% We will use LDAP for examples throughout the section. It is best to
% give a brief introduction to it here.

% LDAP material may be better in the Background section?

\emph{LDAP}~\cite{Sermersheim2006} directory servers are commonly used
in enterprise environments to store and maintain employee contact
information and credentials. We use LDAP directory servers as an
example service which requires emulation. It is well suited to this
task as it is non-trivial, requiring some sophistication in the
modelling, and is widely deployed in enterprise environments targeted
by our approach.

There are 11 different LDAP operations in total falling into three
different categories: \emph{authentication}, \emph{searching} and
\emph{modification}. To conserve space we consider a single operation
from each category: 
\begin{itemize}
\item {\sf bind}: The operation {\sf bind} is from the authentication
  category. It is used by a client to connect to an LDAP directory
  using some authentication credentials.  A {\sf bind request}
  results in a {\sf bind response} from the LDAP server.  The {\sf
    bind response} indicates whether the corresponding {\sf bind
    request} was successful or not. After successfully binding to an
  LDAP server, search and modification operations for the client will
  be enabled.
\item {\sf search}: The operation {\sf search} allows a bound client
  to search an LDAP directory. The client issues a {\sf search
    request} which contains a rich description of the search
  criteria. Searches may be restricted to certain levels of the
  directory tree, time and size limits may be specified on the
  directories responses, and search filters can be used to build
  powerful predicate based search criteria. Each {\sf search request}
  issued by a client is matched by zero or more {\sf search result}
  entries from the LDAP server and is finalised by a single search
  result done.
\item {\sf add}: Finally, the operation {\sf add} allows a bound
  client to insert an entry into an LDAP directory. An {\sf add
    request} from a client is matched by a single {\sf add response}
  from the server, indicating whether the corresponding request was
  successful or not.
\end{itemize}

